Synchronizing Deterministic Push-Down Automata Can Be Really Hard

The question if a deterministic finite automaton admits a software reset in the form of a so-called synchronizing word can be answered in polynomial time. In this paper, we extend this algorithmic question to deterministic automata beyond finite automata. We prove that the question of synchronizability becomes undecidable even when looking at deterministic one-counter automata. This is also true for another classical mild extension of regularity, namely that of deterministic one-turn push-down automata. However, when we combine both restrictions, we arrive at scenarios with a PSPACE-complete (and hence decidable) synchronizability problem. Likewise, we arrive at a decidable synchronizability problem for (partially) blind deterministic counter automata. There are several interpretations of what synchronizability should mean for deterministic push-down automata. This is depending on the role of the stack: should it be empty on synchronization, should it be always the same or is it arbitrary? For the automata classes studied in this paper, the complexity or decidability status of the synchronizability problem is mostly independent of this technicality, but we also discuss one class of automata where this makes a difference.

==> DVPDA-arb-construction.tex <==
\begin{figure}
	\scalebox{0.845}{
	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,semithick,state/.style={circle, draw, minimum size=.9cm}]
	
		\draw[fill=gray!20,draw=white] (-1,-4.8) rectangle (12, -3.2);
		\node at (3, -4.5) {$A$};
		
		\draw[fill=gray!40,draw=gray!20] (8,-4) ellipse (3.3cm and .6cm);
		\node at (5.5, -4) {$S$};
	
		\node[state] (1'') {$p''$};
		\node[state] (1') [below of=1''] {$p'$};
		\node[state] (1) [below of=1'] {$p$};
		
		\node[state] (2'') [right of=1''] {$q''$};
		\node[state] (2') [below of=2''] {$q'$};
		\node[state] (2) [below of=2'] {$q$};
		\node [right of=2] {$\dots$};
		\node [right of=2'] {$\dots$};
		\node [right of=2''] {$\dots$};
		
		\node[state] (3'') at (6.5, 0) {$r''$};
		\node[state] (3') [below of=3''] {$r'$};
		\node[state] (3) [below of=3'] {$r$};
		
		\node[state] (4'') [right of=3''] {$s''$};
		\node[state] (4') [below of=4''] {$s'$};
		\node[state] (4) [below of=4'] {$s$};
		\node (S) [right of=4] {$\dots$};
		\node [right of=4'] {$\dots$};
		\node (S'') [right of=4''] {$\dots$};
		
		\node[state] (fin) at (12.5, -2) {$q_{\text{fin}}$};
		\node[state] (stall) [above of=fin]{$q_{\text{stall}}$};
		
	
		
		\path
		(1'') edge [bend left=10] node [pos=0.35] {$a, \push(p)$} (1')
		(1') edge [bend left=10] node [pos=0.35]{$a, \push(p)$} (1)
		(1) edge [loop below] node {$a, \push(p)$} (1)
		(1') edge [bend left=10] node {$b, \pop(p)$} (1'')
		(1) edge [bend left=10] node {$b, \pop(p)$} (1')
		(1'') edge [loop above] node {$b, \pop(p)$} (1'')
		%		
		(2'') edge [bend left=10] node {$a, \push(p)$} (2')
		(2') edge [bend left=10] node {$a, \push(p)$} (2)
		(2) edge [loop below] node {$a, \push(p)$} (2)
		(2') edge [bend left=10] node [pos=0.35]{$b, \pop(p)$} (2'')
		(2) edge [bend left=10] node [pos=0.35]{$b, \pop(p)$} (2')
		(2'') edge [loop above] node {$b, \pop(p)$} (2'')
		%
		%
		(3'') edge [bend left=10] node [pos=0.35] {$a, \push(p)$} (3')
		(3') edge  node [pos=0.35]{$a, \push(p)$} (3)
		(3) edge [loop below] node {$a, \push(p)$} (3)
		(3') edge [bend left=10] node {$b, \pop(p)$} (3'')
		(3) edge [bend right=10] node [pos=0.75, above] {$b, \pop(Q)$} (fin)
		(3'') edge [loop above] node {$b, \pop(p)$} (3'')
		%		
		(4'') edge [bend left=10] node {$a, \push(p)$} (4')
		(4') edge  node {$a, \push(p)$} (4)
		(4) edge [loop below] node {$a, \push(p)$} (4)
		(4') edge [bend left=10] node [pos=0.35]{$b, \pop(p)$} (4'')
		(4) edge [bend right=10] node [pos=0.75,below]{$b, \pop(Q)$} (fin)
		(4'') edge [loop above] node {$b, \pop(p)$} (4'')
		%
		(1'') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (1'')
		(1') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (1')
		(3'') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (3'')
		(3') edge [loop left] node [pos=0.3] {$\Sigma_{\text{int}}$} (3')
		(2'') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (2'')
		(2') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (2')
		(4'') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (4'')
		(4') edge [loop right] node [pos=0.7] {$\Sigma_{\text{int}}$} (4')
		%
		(S) edge [bend right=10] node [pos = 0.3, right] {$b, \pop(Q)$}(fin)
		(fin) edge [bend right, color=red] node [left,pos=0.2] {$b, \pop(Q)$} (12, -1)
		(stall) edge [bend right,color=red] node [left, pos=0.2] {$b, \pop(Q)$} (12, 1)
		(fin) edge [bend left=10] node[above] {$b, \pop(\bot)$} (4'')
		(stall) edge [bend right=20] node [above,pos=0.7] {$b, \pop(\bot)$} (4'')
		%
		(fin) edge [loop right] node {$a, \push(F)$} (fin)
		(stall) edge [loop right] node {$a, \push(F)$} (stall)
		(stall) edge [bend left=10] node {$b, \pop(F)$} (fin)
		(fin) edge [bend left=10] node[pos=0.7] {$b, \pop(F)$} (stall)
		;
	\end{tikzpicture}
}
\caption{Illustration of the DVPDA $M$ in the proof of Theorem~\ref{thm:DVPA-Arb-PSPACE}. In a transition $\push(q)$ means that the stack symbol $q$ is pushed on top of the stack with this transition. Similarly, $\pop(q)$ means that the stack symbol $q$ is popped from the stack with this transition. The transitions drawn in red lead to the annotated state $q''$ if the letter $q$ is popped from the stack. For reasons of clarity and comprehensibility, the following transitions are \emph{not} drawn: For $q \in Q, q'\in Q', q''\in Q''$ $\delta'(\{q, q', q''\}, b, p)$ for $q \neq p$; 
$\delta'(\{q_{\text{fin}}, q_{\text{stall}}\}, b, Q)$;
$\delta'(Q \cup Q' \cup Q'', b, \bot)$;
$\delta'(Q, \Sigma_{\text{int}})$.
}
\label{fig:DVPDA-Arb}
\end{figure}
